A Novel Computational Thermodynamics Framework with Intrinsic Chemical Short-Range Order

Chemical short-range order (SRO) provides new opportunities for tuning alloy properties, but conventional computational thermodynamics frameworks such as CALPHAD, based on Bragg-Williams mean-field approximations, cannot properly describe SRO or order-disorder transformations in multicomponent ($\geq$3) alloys. First-principles approaches combined with the cluster variation method (CVM) or cluster expansion method (CEM) can capture SRO but suffer from high computational cost. Here we present a hybrid CVM-CALPHAD framework with a thermodynamic solid solution model named as FYL-CVM, enabled by the Fowler-Yang-Li (FYL) transform to reduce the number of variables required in free-energy minimization. This achieves efficient modeling of SRO in multicomponent systems within the CALPHAD formalism. Benchmark tests on fcc AB binaries show that FYL-CVM reproduces CVM phase diagrams with much higher efficiency, while non-configurational contributions from vibrational, elastic, and electronic terms are also incorporated to capture their physical effects on order-disorder boundaries. Applied to the Cu-Au system, this method produces phase diagrams with experimental data in an efficient parameterization and elucidates the temperature-composition dependence of SRO parameters via the SRO diagram. Its applicability to ternary alloys is also demonstrated for the Cu-Au-Ag system. Overall, this framework strikes a balance between accuracy and efficiency, extends CALPHAD to account for chemical SRO, and enables a comprehensive physics-informed modeling of ordering phenomena. (This dissertation was submitted to the University of Virginia in 2023 as the author's doctoral research. For the original complete abstract, please refer to the PDF version.)

==> deletedpart4bignamesection.tex <==
\\Along my long journey, I want to thank many other big names over the world for helping me build up my taste in science but not only science. What I am trying to pursue is to explore the “scattering pattern” while fundamental mathematics “interact” and “resonate” with the real world or say, applied mathematics. When I entered my undergraduate school, I kept my high school interests in pure mathematics and still wanted to become a pure mathematician but not the saber to attack real world challenge with mathematics as the Excalibur. I was influenced by the great Shing-Tung Yau at that age, and his stories inspired my diligence in learning mathematics. After I entered undergraduate school, I learned both intuitive style and constructive style mathematics. The intuitive style might be influenced by Professor Vladimir Arnold’s important talk: \textit{On Math Teaching}.
\\But I also learned a lot of Boubaki style’s or say constructive style work, they basically have three steps: \textit{"define an algebraic structure, prove the structure can depict the object we want, find an example to prove this structure exist"}. Although in the great Michael Atiyah’s talk: \textit{Mathematics in the 20th century}, they are separated into two different styles of mathematicians. From my perspective, they could be consistent with each other. One of the typical coherent consistencies happened in the great Zorich’s textbook \textit{mathematical analysis}, which provide lots of interesting example to combine the abstract definition of mathematical structure and concrete but impressive application in physics and industry. My favor of this well-coherent style work later was strengthed by the great Elias M. Stein’s four textbooks in analysis and several articles from Professor Liang Kong.
\\When I learned the Riemann Geometry textbook written by professor Hung-Hsi Wu, I learned how to consider mathematics more fundamentally and think highly of the motivation to develop a theory. The motivations and the applications of a technique could help us to see the connection across the research domain. I also generally learned how to make some “observations” mathematically and finally noticed that what many mathematicians did has nothing difference from what many experimentalists did, they are all the same. It’s all about finding out some interesting and novel “pattern”, experimentalists do this through some device while mathematicians do this through some mathematical derivation. There are some similar statements in the \textit{impression of mathematics} written by professor Kunihiko Kodaira, and of course, Vladimir Arnold’s talk. From this perspective, I do see the strong connection between the practical application and the theoretical thought while starting to believe the power of the integration between the abstract deep mathematical world and the practical real world.
\\When I came to Hangzhou to participate in the Yau’s mathematics competition, I took part in all analysis track, geometry track, and the applied mathematics track. I was attracted by the problems in applied mathematics track while I was reading professor Chia-Chiao Lin’s bible in applied mathematics in the meantime. Professor Lin has lots of interesting articles about the aim and methods of applied mathematics, which could be considered as a kind of paradigm to deal with concrete scientific and engineering problems in a mathematical style. It’s general and diverse while it could be considered as a bridge to connect every discipline from the most abstract mathematical world. Professor Lin himself shifted his research interests from fluid mechanics to astrophysics and finally to biophysics during his whole life. I really respect this exploration: staying in one domain for a lifelong career is a little bit boring for me. I feel like this may come from the influence of one of the greatest entrepreneurs in my mind, Mr. Steve Jobs. I was impressed by his creativity when I was a high school student, and \textit{stay hungry, stay foolish}. 
\\During the final two years of my undergraduate years, I got some physics training from professor Mingda Li just through email and finally published my first work within quantized dislocation, while at that time I don't know too much of materials science/physics but keep presenting my mathematical skills. I feel like this is not enough and gradually shifted myself from pure mathematics to applied mathematics.
\\Then I was fully influenced by professor Chen-Ning Yang during my graduate school, as his master thesis is the foundation of this dissertation. Although he is totally a genius, I learned how he considered problems and his taste through his representative work, presentations and talks. Perhaps one of the most famous public presentations which involved a large debate is about his statement \textit{"the party is over”} for particle physics, but I gradually got his meaning and it might be more close to the content within \textit{The Structure of Scientific Revolutions} by Thomas Kuhn. This actually highly influenced me during my graduate school years, while another highly influenced event is led by professor Weinan E. It also reminds me to be more sensitive to consider which solvable problem would become promising in the future, since perhaps I personally feel like the timing might be more important than niche in some case. The other most important three articles/talks in my mind are his \textit{beaty and physics}, \textit{my experience of study and research}, and \textit{prospect and learning method of physics}. It is Dr. Huitao Shen’s article motivated me to Yang’s \textit{beauty and physics}. In Dr. Shen’s opinion, it’s about how to coherently combine the beauty of mathematical format and the beauty of coincidence between theory and experiments. It’s all about a kind of trinity: experimental results, physical essence, mathematical form. In my understanding, it’s a kind of three-level expansion along the concrete $\to$ abstract direction, and they should be coherently corresponding to each other. It makes me consider why Yang always could catch the timing, as he could always expand himself on the fundamental level to catch the essence, whether through catching the essence in time to catch the milestone work or through catching the essence in structure to take mathematics to lead the intuition.
\\Finally, I want to mention and tribute to professor Weinan E and Dr. Linfeng Zhang as the end of the “big name” section for the acknowledgement. Professor E is the hero in my heart who defines the “new era” of applied mathematics to integrate all first-principles model, data-driven method and algorithms to explore the connection between mathematical world and real world. Another thing I learned from them is to be “problem-driven”: applied mathematics is very broad, you would learn the very general method but have to concentrate on some concrete problem to find the direction to avoid the lost. My thesis could be considered as a small piece of tribute to him to combine the fundamental statistical model for data-driven computational thermodynamics with the corresponding algorithms focusing on the chemical short-range order in solid solution phase. Dr. Linfeng Zhang is trying to build up a brilliant company to combining deep learning and molecular dynamics to explore the way to connect academia and industry to achieve a positive feedback loop through an applied mathematics way. Their courage of the exploration and brave heart really inspired me. When Dr. Linfeng Zhang brings \textit{The Alchemist} to express his wish for his company, in which Paulo Coelho's masterpiece depicts the mystical story of Santiago, I feel like all this connects. So I also want to share my respect to Ya Ge who brought her \textit{The Alchemist} and care to me ten years ago when I was a high school student.

==> modifiedPart.tex <==
\def\titlepage{
      \thispagestyle{empty}
  \begin{center}
  \MakeUppercase{\@title}\\
  \vfill
  \rm \@author\\
   \@homeaddress\\
   \bigskip
   {\noindent \@firstpriordegree , \@firstpriorinstitution , \@firstpriordate \\}
  %IF there is a 2nd prior degree
   \ifbool{@2degrees}{\noindent \@secondpriordegree , \@secondpriorinstitution , \@secondpriordate \\}{}

\vfill

    {\noindent A \@thesis\ submitted to the Graduate Faculty \\ 
    of the \@institution\ in Candidacy for the Degree of \\}

     \@degree \\
\bigskip
     Department of \@program \\
\vfill
    \@institution\\
    \@graddate\\
\vfill
  \begin{flushright}
  \begin{minipage}{0.35\textwidth}
    \noindent \@advisor, \ifbool{@coad}{Co-c}{C}hair \\
    \ifbool{@coad}{\@coadvisor, Co-chair\\}{}
    \ifbool{@1st}{\@secondmember\\}{}
    \ifbool{@2nd}{\@thirdmember\\}{}
    \ifbool{@3rd}{\@fourthmember\\}{}
    \ifbool{@4th}{\@fifthmember\\}{}
    \ifbool{@5th}{\@sixthmember\\}{}
  \end{minipage}
  \end{flushright}
  \vfill
%   \includepdf[pages={2-3}]{CoverNApproval} 



  \end{center}
%\clearpage
%UVA GSAS says copyright page should be numbered
%\pagestyle{empty} % Suppresses page numbers for copyright page.

%Count the title page in the numbering, even though it is not numbered
\addtocounter{page}{1}
\vspace*{\fill}
%\includegraphics[height=2cm]{example-image}

Copyright \textcopyright\ \the\year{}, \@author\ 

\clearpage
  \newpage % This applies to the numbering of the front matter.
  %\addtocounter{page}{1} 
}
